On the Generalization and Adaptation Ability of Machine-Generated Text Detectors in Academic Writing

The rising popularity of large language models (LLMs) has raised concerns about machine-generated text (MGT), particularly in academic settings, where issues like plagiarism and misinformation are prevalent. As a result, developing a highly generalizable and adaptable MGT detection system has become an urgent priority. Given that LLMs are most commonly misused in academic writing, this work investigates the generalization and adaptation capabilities of MGT detectors in three key aspects specific to academic writing: First, we construct MGT-Acedemic, a large-scale dataset comprising over 336M tokens and 749K samples. MGT-Acedemic focuses on academic writing, featuring human-written texts (HWTs) and MGTs across STEM, Humanities, and Social Sciences, paired with an extensible code framework for efficient benchmarking. Second, we benchmark the performance of various detectors for binary classification and attribution tasks in both in-domain and cross-domain settings. This benchmark reveals the often-overlooked challenges of attribution tasks. Third, we introduce a novel attribution task where models have to adapt to new classes over time without (or with very limited) access to prior training data in both few-shot and many-shot scenarios. We implement eight different adapting techniques to improve the performance and highlight the inherent complexity of the task. Our findings provide insights into the generalization and adaptation ability of MGT detectors across diverse scenarios and lay the foundation for building robust, adaptive detection systems. The code framework is available at https://github.com/Y-L-LIU/MGTBench-2.0.

==> edit_wiki_prompt.tex <==
\begin{tcolorbox}[colback=orange!10,
                  colframe=orange!70,
                  width=\columnwidth,
                  fonttitle=\bfseries\centering, % Center the title
                  coltitle=black, 
                  arc=3mm, auto outer arc,
                  before=\vspace{2pt},  % Reduces space before the box
                  after=\vspace{3pt},
                  boxsep=1pt,
                  left=2pt,
                  right=2pt,
                  title=Prompt Template for Wiki Text
                 ]
\small
\begin{tabularx}{\linewidth}{X}
    % \toprule
    <\underline{Background}>: \\
    Please act as an expert wiki editor and revise the
    wiki content from the perspective of a wiki editor
    to make it fluent and elegant. Here are the specific requirements: \\
    1. You should provide accurate and comprehensive information.
       Use reliable sources and cross-check your information to ensure its accuracy. \\
    2. Wiki articles should be neutral and unbiased. Avoid expressing personal opinions
       or promoting a particular viewpoint. Instead, present all relevant 
       information and let the readers form their own opinions. \\
    3. Your writing should be clear and easy to understand. Avoid using complex sentences 
       and unnecessary words. Remember, your goal is to convey information, not to 
       showcase your vocabulary. Please only include the written wiki page in your answer. \\
    Here is the original wiki page: \\
    <\underline{text}>: //to-be-polished text \\
    % \bottomrule
\end{tabularx}
\end{tcolorbox}
